Bounding Stochastic Safety: Leveraging Freedman's Inequality with Discrete-Time Control Barrier Functions

When deployed in the real world, safe control methods must be robust to unstructured uncertainties such as modeling error and external disturbances. Typical robust safety methods achieve their guarantees by always assuming that the worst-case disturbance will occur. In contrast, this paper utilizes Freedman's inequality in the context of discrete-time control barrier functions (DTCBFs) and c-martingales to provide stronger (less conservative) safety guarantees for stochastic systems. Our approach accounts for the underlying disturbance distribution instead of relying exclusively on its worst-case bound and does not require the barrier function to be upper-bounded, which makes the resulting safety probability bounds more directly useful for intuitive safety constraints such as signed distance. We compare our results with existing safety guarantees, such as input-to-state safety (ISSf) and martingale results that rely on Ville's inequality. When the assumptions for all methods hold, we provide a range of parameters for which our guarantee is stronger. Finally, we present simulation examples, including a bipedal walking robot, that demonstrate the utility and tightness of our safety guarantee.

==> Old_Stuff/issf.tex <==
\begin{align}
    \hline \nonumber 
\end{align}


For the stochastic version, consider the normalized function $\tilde{h}(\mb{x}) = \frac{1}{\frak{L}\Vert \mb{d} \Vert_\infty}h(\mb{x})$, so we know almost surely that $\tilde{h}(\mb{x}_{k+1}) \geq \E[\tilde{h}(\mb{x}_{k+1}) | \F_{k}] - 1$. So we can apply our thereom again to know that: 
\begin{align}
    P_u(K, \mb{x}_0) \leq    
        & \left( \left(\frac{\sigma^2}{\alpha^K h_0 + \sigma^2}\right)^{\alpha^K h_0 + \sigma^2 } \left( \frac{K}{K - \alpha^Kh_0}\right)^{K - \alpha^Kh_0}\right)^{\frac{K}{K + \sigma^2}} \mathds{1}_{\{\alpha^Kh_0 \leq K\} } 
\end{align}
Alternatively, you can get the bound on $\C_\delta $ in probability which just requires shifting the zero for the definition of $W_k = - \alpha^{K-k}\tilde{h}(\mb{x}_k) + \alpha^K(\tilde{h}(\mb{x}_0) + \frac{c}{1 - \alpha})  $ where $c\in [0, \frak{L}_h \Vert \mb{d} \Vert_\infty]$ is the relevant levelset. 
\begin{align}
    P_u(K, \mb{x}_0) \leq    
        & \left( \left(\frac{\sigma^2}{\alpha^K (\tilde{h}_0 + \frac{c}{1-\alpha}) + \sigma^2}\right)^{\alpha^K  (\tilde{h}_0 + \frac{c}{1-\alpha})  + \sigma^2 } \left( \frac{K}{K - \alpha^K (\tilde{h}_0 + \frac{c}{1-\alpha}) }\right)^{K - (\tilde{h}_0  + \frac{c}{1 - \alpha})}\right)^{\frac{K}{K + \sigma^2}} \mathds{1}_{\{\alpha^K (\tilde{h}_0 + \frac{c}{1-\alpha})  \leq K\} } 
\end{align}

\clearpage 


==> Old_Stuff/old_doobs_decomp_stuff.tex <==

\section{Doob's Decomposition}

\begin{definition}[Filtration]
    Let $(\Omega, \cal{F}, \P)$ be a probability space and let $I$ be an index set. For every $i \in I$, let $\cal{F}_i$ be a sub-$\sigma$-algebra of $\cal{F}$. 
    Then 
    \begin{align}
        (\cal{F}_i)_{i\in I}
    \end{align}
    is called a \textit{filtration} if $\cal{F}_k\subseteq \cal{F}_\ell$ for all $k \leq \ell$, 
\end{definition}

\begin{theorem}[Doob's Decomposition Theorem]
Let $(\Omega, \cal{F}, \P)$ be a probability space, $I = \{ 0, 1, \dots, N\} $ for $N \in \mathbb{N}$. Let $(\cal{F}_n)_{n\in I}$ be a filtration of $\cal{F}$ and $X = (X_n)_{n \in I}$ an adapted stochastic process with $\E [ \vert X_n \vert ] \leq \infty $ for all $n \in I$. Then there exists a martingale $M = (M_n)_{n \in I} $ and an integrable predictable process $A = (A_n)_{n \in I} $ starting with $A_0 = 0 $ such that $X_n = M_n + A_n $ for every $n \in I$. Here predictable means that $A_n$ is $\cal{F}_{n-1}$-measureable for every $n \in I\setminus \{ 0\} $. This decomposition is almost surely unique. 
\end{theorem}

The unique decomposition of used in Doob's decomposition theorem is: 
\begin{align}
    A_n & = \sum_{k=1}^n \left( \E [X_k ~|~ \cal{F}_{k-1}] - X_{k-1}\right)\\
    M_n & = X_0 + \sum_{k=1}^n \left( X_k - \E[X_k ~|~ \cal{F}_{k-1}] \right) 
\end{align}

\begin{corollary}
    A real-valued stochastic process $X$ is a \textit{supermartingale} if and only if it has a Doob decomposition into a martingale $A$ and an integrable predictable process $M$ that is almost surely decreasing.     
\end{corollary}


\subsection{Application}

Consider the CBF condition: 
\begin{align}
\E [h(\mb{F}(\mb{x}_k) + \mb{d}_k) ~|~ \cal{F}_{k}] \geq \alpha h(\mb{x}_k) 
\end{align}
where the disturbance is a $\F_{k+1}$-measurable random variable $\mb{d}_k\sim\cal{D}(\mb{x}_k)$. 

Define the supermartingale: 
\begin{align}
    W_k = -\alpha^{-k}h(\mb{x}_k) + h(\mb{x}_0) 
\end{align}

Using Doob's martingale decomposition we define the predictable $\F_{k-1}$-measurable supermartingale: 
\begin{align}
    A_k &= \sum_{i=1}^k \left( \E[W_k ~|~ \F_{k-1}] - W_{k-1} \right) \\
    & = \sum_{i=1}^k \left( -\alpha^{-k} \E [~ h(\mb{x}_k) ~|~ \F_{k-1}~] + \alpha^{-(k-1)} h(\mb{x}_{k-1}) \right) \nonumber\\
    & = \sum_{i=1}^k -\alpha^{-k}\left(\E [~ h(\mb{x}_k) ~|~ \F_{k-1}~] - \alpha h(\mb{x}_{k-1}) \right) \nonumber
\end{align}

According to Doob's Decomposition Theorem, this defines the martingale: 
\begin{align}
    M_k & \triangleq W_k - A_k \\
    & = - \alpha^{-k} h(\mb{x}_k) + h(\mb{x}_0)  \\
    & \quad \quad + \sum_{i=1}^k \alpha^{-k}\left(\E [~ h(\mb{x}_k) ~|~ \F_{k-1}~] + \alpha h(\mb{x}_{k-1}) \right) \nonumber 
\end{align}

This leads to the martingale differences: 
\begin{align}
    M_k - M_{k-1} & = W_k - \E [W_{k}~|~ \cal{F}_{k-1}]\\
    & = -\alpha^{-k} \left( h(\mb{x}_k) - \E[h(\mb{x}_k) ~|~ \cal{F}_{k-1}] \right) 
\end{align}
This needs to be upper bounded by 1, so we require that: 
\begin{align}
    h(\mb{x}_k) - \E[h(\mb{x}_k) ~|~ \cal{F}_{k-1}] \geq -\alpha^k
\end{align}

This can be used to produce a risk-sensitive bound on the event:  
\begin{align}
    & \left\{ \sup_{k \leq K } M_k \leq \lambda \right\}\\
    & \;\; = \{ \sup_{k\leq K} - \alpha^{-k} h(\mb{x}_k) + h(\mb{x}_0) \\
    & \quad \quad \quad \quad \quad + \sum_{i=1}^K \alpha^{-k} ( \E[h(\mb{x}_k ~|~ \F_{k-1}]) - \alpha h(\mb{x}_{k-1})) \leq \lambda \} \nonumber  
\end{align}

\subsection{Doob's Decomposition for $c$-martingales}

Consider the $c$-barrier function condition \textit{a la} Steinhardt and Tedrake: 
\begin{align}
    \E [h(\mb{x}_{k+1} ) ~|~ \F_{k}] \geq h(\mb{x}_k) - c \label{eq:c-barrier_cond}
\end{align}
We then define a candidate function: 
\begin{align}
    W_{k} \triangleq - h(\mb{x}_k) - k c + h(\mb{x}_0). 
\end{align}
This candidate function has two nice properties: 
\begin{itemize}
    \item $W_0 = -h(\mb{x}_0) + 0 + h(\mb{x}_0)  = 0 $, 
    \item $W_k$ is a super-martingale:  
    \begin{align}
        \E[W_{k+1} ~|~ \F_{k}]  & = \E[-h(\mb{x}_{k+1}) ~|~ \F_{k}]- (k+1)c + h(\mb{x}_0) \nonumber \\
        & \leq -h(\mb{x}_{k}) + c - (k+1) c + h(\mb{x}_0) \nonumber \\
        & = - h(\mb{x}_k) - kc + h(\mb{x}_0) = W_k. 
    \end{align}
\end{itemize}

We can now decompose $W_k$ using Doob's decomposition into a $\F_{k-1}$-predictable supermartingale, $A_k$,  and a martingale, $M_k$.

First we define $A_k$ and show that it is a super-martingale: 
\begin{align}
    A_k & \triangleq \sum_{k=1}^n \left( \E [ W_k ~|~ \F_{k-1} ] - W_{k-1} \right) \\
    \E[ A_{k+1} ~|~ \F_{k}] & = \E[W_{k+1} ~|~ \F_{k}] - W_k + A_k\\
    & \leq  A_k 
\end{align}

Next we define $M_k$ and show that it is a martingale (and therefore also a supermartingale): 
\begin{align}
    M_k & \triangleq W_k - A_k \\
    \E[M_k - M_{k-1}~ | ~ \F_{k-1} ] & =\E [ W_k - W_{k-1} \\
    & \quad - (\E [W_k ~|~ \F_{k-1}] - W_{k-1}) ~|~ \F_{k-1}] \nonumber \\
    & = 0 
\end{align}


We now make two key assumptions: 
\begin{assumption}[Bounded Predictable Quadratic Variation]\label{assp:bounded_pred_quad_var}
    We assume that the predictable quadratic variation of $M_k$, defined as: 
    \begin{align}
        \langle M \rangle_k = \sum_{i = 1}^k \E [ \left( M_i - M_{i-1}\right)^2 ~|~ \F_{i-1}]
    \end{align}
    is upper-bounded by $\sigma^2>0$, i.e. $\langle M \rangle_k \leq \sigma^2$. 
\end{assumption}

\begin{assumption}[Upper Bounded Martingale Differences]\label{assp:bounded_mart_diff} 
    We assume that the martingale differences for $M_k$ are upper-bounded by $ 1$: 
    \begin{align}
        M_k - M_{k-1}  \leq 1 
    \end{align}
\end{assumption}
This assumption is equivalent to assuming that $h(\mb{x}_k) \geq \E[h(\mb{x}_k) ~|~ \F_{k-1}] - 1  $. Intuitively, this requires that the true safety value cannot be less than one less than the expected safe value. 

These assumptions allow us to apply the main theorem from \textit{Hoeffding's Inequality for Supermartingales} by Xiequan Fan, et al (2012) which is restated here: 
\begin{theorem}
    Assume that $(M_{k} - M_{k-1}, \F_k)_{k=1, \dots, K }$ are supermartingale differences satisfying $(M_k - M_{k-1})\leq 1 $. Then, for any $\lambda \geq 0 $ and $\sigma > 0 $, 
    \begin{align}
        \P \{ \max_{k \leq K } M_k \geq \lambda \textup{ and } \max_{k \leq K }\langle M \rangle_k \leq \sigma^2 \} \leq H_{K}(\lambda, \sigma), 
    \end{align}
    where 
    \begin{align}
        H_K(\lambda, \sigma ) & = \left\{ \left( \frac{\sigma^2}{\lambda + \sigma^2}\right)^{x + \sigma^2}\left( \frac{K}{K - \lambda} \right)^{n - x}\right\}^{\frac{n}{n+ \sigma^2}} \mathds{1}_{\left\{ \lambda \leq K \right\} }  
    \end{align}
    with the convention that $(+\infty)^0 = 1 $ (which applies when $\lambda = K$). 
\end{theorem}

Using this theorem we can apply it to our $c-$barrier function problem to arrive at this theorem: 
\begin{theorem}
    If the system satisfies condition \eqref{eq:c-barrier_cond} and assumptions \ref{assp:bounded_pred_quad_var} and \ref{assp:bounded_mart_diff} hold, then the probability of becoming unsafe satisfies this bound: 
    \begin{align}
        \P \left\{ \right\} 
    \end{align}
\end{theorem}


==> bonus/basic_prob_background.tex <==

\subsection{Basic Probability Background}

\begin{definition}[Sample Space]
    The \textit{sample space} is a fixed set $\Omega$ whose elements, $\omega$, are called ``sample point'' or ``outcomes''.  
\end{definition}



\begin{definition}[$\sigma$-algebra]
A collection $\F$ subsets of $\Omega$ is called an \textit{algebra} if: 
\begin{enumerate}
    \item It contains the empty set and whole set $\emptyset \in \F$ and $\Omega \in \F$. 
    \item It is stable under complements: $A \in \F \implies A^c \in \F$. 
    \item It is stable under union and intersection: $A, B \in \F \implies A \cup B \in \F $ and $A \cap B \in \F$. 
\end{enumerate}
The collection $\F$ is a $\sigma$-algebra if it satisfies the stronger condition that it is stable under \textit{countable} unions and intersections: 
\begin{align}
    A_i \in \F \textup{ for each } i \in \mathbb{N} \implies \bigcup_{i=1}^\infty A_i \in \F \textup{ and } \bigcap_{i=1}^\infty A_i \in \F
\end{align}
\end{definition}


\begin{definition}[Measure]
    Let $(\Omega, \F)$ be a samp-le space, equipped with a $\sigma$-algebra. A \textit{measure} $\mu: \F \to [0, \infty]$ is a set function that satisfies: 
    \begin{enumerate}
        \item $\mu(\emptyset ) = 0 $
        \item If $A_i \in \F $ for $i \in \mathbb{N}$ is a disjoint family of sets, then the meausre of the union is the sum of the measures: 
        \begin{align}
            \mu \left(\bigcup_{i=1}^\infty A_i \right) = \sum_{i=1}^\infty \mu(A_i).  \nonumber 
        \end{align}
        \item If $\mu$ also satisfies: $\mu(\Omega) = 1 $, then we call it a ``probability measure''. 
    \end{enumerate}
\end{definition}

\begin{definition}[Probability Space]
    A probability space is a triple $(\Omega, \F, \mu) $ where 
    \begin{itemize}
        \item $\Omega$ is the sample space 
        \item $\F $ is a $\sigma$-algebra on $\Omega$
        \item $\mu$ is a probability measure on $(\Omega, \F) $
    \end{itemize}
\end{definition}

\begin{definition}[Borel $\sigma-$algebra]
    Fix the sample space $\Omega = \R$. Consider the class $\mathscr{C}$ of closed half-lines: 
    \begin{align}
        \mathscr{C} = \{(-\infty, a] ~|~ a \in \R \}. 
    \end{align}
    The Borel $\sigma-$algebra on $\R$ is the class: 
    \begin{align}
        \scr{B}\triangleq \scr{B}(\R) \triangleq \sigma(\scr{C}) = \sigma (\{(-\infty, a] ~|~ a \in \R\}) 
    \end{align}
\end{definition}

\begin{definition}[Measurable Function]
    Let $(\Omega, \F) $ be a measurable space composed of a sample space, $\Omega$, and a $\sigma-$algebra, $\F$. A function, $f:\Omega \to \R$, is (Borel) measurable when, for any Borel set $B \in \cal{B}(\R) $, the inverse image of $B$ under $f$ is an event. That is, 
    \begin{align}
        f^{-1}(B) \triangleq \{ \omega \in \Omega ~|~ f(\omega) \in B \} \in \F
    \end{align}
\end{definition}

\begin{definition}[Random Variable]
    Let $(\Omega, \F, \P) $ be a probability space. A (real) random variable is a Borel measurable function $X: \Omega \to \R $. 
\end{definition}

\begin{definition}[Distribution] 
    The \textit{law} or \textit{distribution} of the random variable $X$ is the measure: 
    \begin{align}
        \mu(B) \triangleq \P (X^{-1}(B)) 
    \end{align}
    where the measure is defined on the Borel subsets $B$ of $\R$. 
\end{definition}

\begin{definition}[Cumulative Distribution Function]
    The \textit{cumulative distribution function} of a random variable $X$ measures the cumulative probability of $X$ up to the threshold $a \in \R$: 
    \begin{align}
        F_X(a) & \triangleq \P\{ X \leq a \} \\
& \triangleq \P\{ \omega \in \Omega ~|~ X(\omega) \leq a\} \\
& = \P (X^{-1}(-\infty,a]) 
    \end{align}
\end{definition}

\begin{definition}[Lebesgue Integral]
    For a nonnegative measurable function $f$, 
    \begin{align}
        \int f d\mu \triangleq \int_{t = 0 }^\infty \mu \{\omega ~|~ f(\omega) > t \} dt 
    \end{align}
    Properties: linear, positive, monotone, insensitive to null sets (i.e., almost everywhere)
\end{definition}

==> bonus/bounding_delta_and_sigma.tex <==

% We restate this proposition here for reference:
%         \begin{proposition*}
%             If 
%             \begin{align}
%                 & \mb{d}\sim \mathcal{D} \textup{ satisfies } \Vert\mb{d}\Vert\leq d_\textup{max} \textup{ for some } d_{\max} \geq 0, \\
%                 & h:\R^n\to \R \textup{ is globally Lipschitz with } \mathcal{L}_h\geq 0, \\
%                 & \mb{x}_{k+1} = \mb{F}(\mb{x}_k) + \mb{d}_k, \textup{ for some $\mb{F}: \R^n \to \R^n,$}
%             \end{align}   
%             then 
%             \begin{align}
%                 \E[h(\mb{x}_k) ~|~ \mathscr{F}_{k-1} ] - h(\mb{x}_k) & \leq 2\mathcal{L}_hd_{\max}   \triangleq \delta, \\
%                 \textup{Var}(h(\mb{x}_{k+1})~|~ \mathscr{F}_k) & \leq  \mathcal{L}_h^2 d_{\max}^2 \triangleq \sigma^2.
%             \end{align}
%         \end{proposition*}

% \noindent\underline{Proof:}

%     First we bound $\delta$:
%             \begin{align}
%                 \E[h(\mb{x}_k) ~|~ \mathscr{F}_{k-1}] - h(\mb{x}_k) 
%                 & = \mathbb{E}[h(\mb{F}(\mb{x}_{k-1}) + \mb{d}_{k-1}) ~|~\mathscr{F}_{k-1}] - h(\mb{F}(\mb{x}_{k-1}) + \mb{d}_{k-1})   \\
%                 & \leq \mathbb{E}[h(\mb{F}(\mb{x}_{k-1})) + \mathcal{L}_h \Vert \mb{d}_{k-1}\Vert ~|~ \mathscr{F}_{k-1} ] - h(\mb{F}(\mb{x}_{k-1})) + \mathcal{L}_h \Vert \mb{d}_{k-1}\Vert  \\
%                 &  = h(\mb{F}(\mb{x}_{k-1})) - h(\mb{F}(\mb{x}_{k-1}))+  \mathcal{L}_h\mathbb{E}[ \Vert \mb{d}_{k-1}\Vert ]  + \mathcal{L}_h \Vert \mb{d}_{k-1}\Vert\\
%                 & \leq \mathcal{L}_h\mathbb{E}[d_{\max} ] + \mathcal{L}_h d_{\max} = 2\mathcal{L}_hd_{\max}\triangleq \delta.
%             \end{align}
%             To bound $\sigma^2$, note that Lipschitz continuity of $h$ implies that: 
%             \begin{align}
%                 h(\mb{F}(\mb{x}_k)) - \mathcal{L}_h d_{\max} \leq h(\mb{F}(\mb{x}_k) + \mb{d}_k) \leq h(\mb{F}(\mb{x}_k)) + \mathcal{L}d_{\max}.  
%             \end{align}
%             Thus, the distribution of $h(\mb{F}(\mb{x}_k) + \mb{d}_k)$ is bounded at $\mathscr{F}_k$, so we can use Popoviciu's inequality on variances \cite{popoviciu1935equations} to achieve: 
%             \begin{align}
%                 \textup{Var}(h(\mb{F}(\mb{x}_k) + \mb{d} ~|~ \mathscr{F}_{k-1}) \leq \mathcal{L}_h^2d_{\max}^2 \triangleq \sigma^2.
%             \end{align}
% \qed 

% \noindent This proposition has been added to the extended version of our work \cite[Appx. G]{cosner2024bounding} and has been cited in our updated submission.


% Next we present how the bounds for $\delta $ and $\sigma $ were obtained in the case of our motivating bipedal robotics example. A shorter version of this discussion was added to the extended manuscript as \cite[Appx. H]{cosner2024bounding}.

% \noindent \underline{Bounding $\delta$ in the Bipedal Example}

%  The bound (14) can be obtained for the example in our paper by using the given assumptions that $\mathcal{D}$ is uniform on the ball of radius $d_\textup{max}$ and that the matrices $\mb{C}$ and $\mb{D}$ reflect the fact that safety is defined only with respect to position and that the global position and the center-of-mass (COM) position are coupled. These facts give $\mb{C}$ and $\mb{D}$ this structure: 
% \begin{align}
%     \mb{C} = \lmat 1& 0 & 0 & 0& 0 & 0 \\ 0 & 1 & 0 & 0 & 0 & 0\\ 0 & 0 & 0 & 0& 0 & 0\\ 0 & 0 & 0 & 0& 0 & 0\\ 0 & 0 & 0 & 0& 0 & 0\\ 0 & 0 & 0 & 0 & 0 & 0 \rmat, &&  \mb{D} = \lmat 1 & 0 & 0 & 0 \\
%         0 & 1 & 0 & 0 \\
%         1 & 0 & 0 & 0 \\
%         0 & 1 & 0 & 0 \\
%         0 & 0 & 1 & 0 \\
%         0 & 0 & 0 & 1\rmat 
% \end{align}
% In this case we can calculate $\delta$ as: 
% \begin{align}
%     & \mathbb{E}[h(\mb{x}_k) ~|~ \mathscr{F}_{k-1}] - h(\mb{x}_k) \\
%     & =     \mathbb{E}[h(\mb{C}(\mb{A}\mb{x}_{k-1} + \mb{B}\mb{u}_{k-1} + \mb{D}\mb{d}_{k-1})] ~|~ \mathscr{F}_{k-1}] - h(\mb{C}(\mb{A}\mb{x}_{k-1} + \mb{B}\mb{u}_{k-1} + \mb{D}\mb{d}_{k-1}))\\
%     & = \mathbb{E}[\Vert \mb{C}(\mb{A}\mb{x}_{k-1} + \mb{B}\mb{u}_{k-1} + \mb{D}\mb{d}_{k-1} - \bs{\rho}\Vert] ~|~ \mathscr{F}_{k-1}] - \Vert\mb{C}(\mb{A}\mb{x}_{k-1} + \mb{B}\mb{u}_{k-1} + \mb{D}\mb{d}_{k-1} - \bs{\rho}\Vert\\
%     & \leq \Vert \mb{C}(\mb{A}\mb{x}_{k-1} + \mb{B}\mb{u}_{k-1}) - \bs{\rho} \Vert +  \mathbb{E}[ \Vert \mb{C}\mb{D}\mb{d}_{k-1} \Vert]] - \Vert\mb{C}(\mb{A}\mb{x}_{k-1} + \mb{B}\mb{u}_{k-1}  - \bs{\rho})\Vert + \Vert  \mb{C}\mb{D}\mb{d}_{k-1}\Vert\\
%     & = \mb{E}[\Vert \mb{C} \mb{D} \mb{d}_{k-1} \Vert] + \Vert \mb{C} \mb{D} \mb{d}_{k-1}\Vert \\
%     & \leq \mb{E}[\Vert \mb{C} \mb{D} \mb{d}_{k-1} \Vert] + d_\textup{max}\label{eq:E_on_ball}\\
%     & = \int_{\mathcal{B}_{d_\textup{max}}(0)} \frac{1}{\pi d^2_\textup{max}} \Vert \mb{C} \mb{D} \mb{d}_{k-1} \Vert d\mb{d}_{k-1} + d_\textup{max}\\
%     & = \int_{0}^{2\pi}\int_0^{d_\textup{max}}\frac{r^2}{\pi d^2_{\textup{max}}} dt d\theta + d_\textup{max}  = \frac{2}{3}d_\textup{max} + d_\textup{max} = \frac{5}{3}d_\textup{max} \triangleq \delta. 
% \end{align}
% where we use the triangle inequality and then calculate the expectation in \eqref{eq:E_on_ball} exactly on the ball $\mathcal{B}_{d_\textup{max}}(0)\subset \R^2 $ using a coordinate transform to produce a less conservative bound. 

% \noindent \underline{Bounding $\sigma^2$ in the Bipedal Example}

% Similarly we can bound $\sigma^2$ for our bipedal example using the structure of the problem and thus resulting in a tighter bound than the one from the one from the proposition. 

% To do this, consider some constant vector $\mb{a} \in \R^2$ and random vector $\mb{b} \in \R^2$ that is uniformly distributed on the ball of radius $\mb{d}_\textup{max}$, i.e. $\mathcal{B}_{d_{\textup{max}}}(0)$. 

% First, we will lower-bound $\E[\Vert \mb{a} - \mb{b}\Vert]^2$ using Jensen's inequality given the convexity of the 2-norm: 
% \begin{align}
%     \E [\Vert \mb{a} - \mb{b} \Vert ]% & \geq \E[\big\vert \Vert\mb{a}\Vert - \Vert\mb{b} \Vert\big\vert ] \\
%     & \geq \Vert \mb{a} - \E[\mb{b}] \Vert = \Vert \mb{a} \Vert   \quad (\textup{Jensen's Inequality}) \\
%     \implies \E[\Vert \mb{a} - \mb{b}\Vert]^2 & \geq \Vert \mb{a} \Vert^2
% \end{align}

% % Alternatively, 
% % First, we will lower-bound $\E[\Vert \mb{a} - \mb{b}\Vert]^2$ using Jensen's inequality given the convexity of the 2-norm: 
% % \begin{align}
% %     \E [\Vert \mb{a} - \mb{b} \Vert ]% & \geq \E[\big\vert \Vert\mb{a}\Vert - \Vert\mb{b} \Vert\big\vert ] \\
% %     & \geq \E[\vert  \Vert \mb{a} \Vert - \Vert \mb{b} \Vert \vert ]  \geq  \vert  \Vert \mb{a} \Vert - \E[\Vert \mb{b} \Vert] \vert    \quad (\textup{Reverse Triangle Inequality}) \\
% %     \implies \E[\Vert \mb{a} - \mb{b}\Vert]^2 & \geq \Vert \mb{a} \Vert^2 - 2\Vert \mb{a} \Vert \E[\Vert \mb{b} \Vert] + \E [ \Vert \mb{b} \Vert]^2
% % \end{align}

% Next, we will bound $\E[\Vert \mb{a} - \mb{b}\Vert^2] $ by using the definition of the 2-norm squared and the linearity of the expectation, 
% \begin{align}
%     % \E[\Vert \mb{a} - \mb{b}\Vert^2 ]& \leq \E[\Vert \mb{a} \Vert^2 + 2 \Vert \mb{a} \Vert\Vert  \mb{b} \Vert + \Vert \mb{b} \Vert^2] \\
%     % & = \Vert \mb{a}^2\Vert + 2 \Vert \mb{a} \Vert \E[\Vert \mb{b} \Vert ] + \E[\Vert \mb{b}\Vert^2]
%     \E[\Vert \mb{a} - \mb{b}\Vert^2 ]& = \E[(\mb{a} - \mb{b})^\top (\mb{a} - \mb{b}) ] = \E[ \mb{a}^\top \mb{a} - 2 \mb{a}^\top \mb{b} + \mb{b}^\top \mb{b}]\\
%     & = \Vert \mb{a} \Vert^2 - 2 \mb{a}^\top \E[\mb{b}] + \E [ \Vert \mb{b} \Vert^2 ] = \Vert \mb{a} \Vert^2 + \E[\Vert \mb{b} \Vert^2]
% \end{align}
% We then use these two bounds, along with a coordinate transform, to calculate the variance. 
% \begin{align}
%     \textup{Var}(\Vert \mb{a} - \mb{b} \Vert) & = \E[\Vert \mb{a} - \mb{b} \Vert^2] - \E[\Vert \mb{a} - \mb{b} \Vert]^2\\
%     & \leq \E[\Vert \mb{a} - \mb{b}\Vert^2 ] - \Vert \mb{a} \Vert^2 \\
%     & =  \Vert \mb{a}\Vert^2  + \E[\Vert \mb{b}\Vert^2]  - \Vert \mb{a} \Vert^2 \\
%     & = \int_0^{2\pi}\int_{0}^{d_\textup{max}} \frac{r^3}{\pi d_\textup{max}^2} drd\theta \\
%     & = \frac{2\pi d_\textup{max}^4}{4 \pi d_\textup{max}^2} = \frac{1}{2}d_{\textup{max}}^2 \triangleq \sigma^2
% \end{align}



==> extended_proofs/comparison_proof.tex <==
\begin{proposition} \label{thm:comparison}
    % Consider some function $h: \R^N \to \R$ that is upper-bounded by $M>0$ with some dynamics that satisfy one of the following cases for some $K \in \mathbb{N}$:

    % \begin{itemize}
    %     \item \textbf{Case (A)}  
    % \begin{align}
    %     \E[~h(\mb{x}_{k+1}) ~|~ \F_{k-1}~] & \geq \alpha h(\mb{x}_k)\\
    %     h(\mb{x}_k) &\geq \E[h(\mb{x}_k)  ~|~ \F_{k-1}] - 1\\
    %     \alpha^K h(\mb{x}_0) &\geq  K\underbrace{(h(\mb{x}_k) - \E[h(\mb{x}_k) |\F_{k-1}])^2}_{\sigma^2 \triangleq} \nonumber  
    % \end{align}
    % for some $\alpha \in (0,1)$. 
    % \item \textbf{Case (B)}
    % \begin{align}
    %     \E[~h(\mb{x}_{k+1}) ~|~ \F_{k-1}~] & \geq h(\mb{x}_k) -c\\
    %     h(\mb{x}_k) &\geq \E[h(\mb{x}_k)~|~ \F_{k-1}] - 1\\
    %     h(\mb{x}_0) - K c  &\geq  K\underbrace{(h(\mb{x}_k) - \E[h(\mb{x}_k) |\F_{k-1}])^2}_{\sigma^2\triangleq} \nonumber 
    % \end{align}
    % for some $c \geq 0 $. 
    % \end{itemize}
    For some $\nu, \lambda, \rho, B > 0 $ and the Lambert-$W$ function\footnote{See Appendix \ref{appdx:comparison} for the definition of the Lambert-$W$ function}, consider the case when
    \begin{align}
        \nu^2  \leq \rho\lambda,  &&  \lambda  \leq B - 1, && \varphi e^\varphi \in [- e^{-1}, 0), &&  B \geq \frac{W_{-1}(\varphi e^\varphi)}{\varphi} \nonumber %W_{-1}(\varphi e^\varphi) \textup{ exists}, \label{eq:lambert_cond} 
    \end{align}
    where $\varphi(\rho)  \triangleq \scriptscriptstyle \ln\left[\left(\frac{\rho}{\rho+1}\right)^{(1 + \rho)}\right] + 1$. If these conditions hold, then:  
    \begin{align}
    H(\lambda, \nu) \leq 1 - \frac{\lambda}{B}.    \label{eq:comparison_thm} 
    \end{align}
\end{proposition}

\begin{proof}%[Proof of Theorem \ref{thm:comparison}:]
    % The Fan, et. al, in \cite{fan2012hoeffding} prove that 
    % \begin{align}
    %     H_K(\lambda, \sigma) \leq \left( \frac{\sigma^2}{\lambda + \sigma^2}\right)^{(\lambda + \sigma^2)}e^\lambda.     
    % \end{align}
    % Therefore, i
    %Let $\Delta:\R_{\geq 0 } \times \R_{\geq 0}  \times \R_{>0} \to \R$ be: %represent the difference between Ville's\eqref{eq:villes_safety_bound} and Hoeffding's \eqref{eq:hoeff_ineq}   safety bounds, i.e.  
    Define %\begin{align}
        $\Delta(\lambda, B, \nu) \triangleq 1 - \frac{\lambda }{B } - H(\lambda, \nu).$  
    %\end{align}
    Thus, if $\Delta(\lambda, B, \nu) \geq 0$, then the desired bound \eqref{eq:comparison_thm} is true. 

    To use our assumption that $\nu^2 \leq \rho \lambda$, we first prove that %over the allowable domain of $\sigma^2 \in(0, \rho \lambda ]$, 
    $\Delta$ is monotonically decreasing in $\nu^2$. Consider $\frac{\partial \Delta }{\partial \nu^2}$:  
    \begin{align}
        \frac{\partial \Delta }{\partial \nu^2} & =  \underbrace{-\frac{e^\lambda}{\nu^2}\left( \frac{\nu^2}{\lambda + \nu^2}\right)^{( \lambda + \nu^2 )}}_{\triangleq a(\lambda, \nu^2) < 0} \underbrace{\bigg( \nu^2 \ln \left( \frac{\nu^2}{\lambda+ \nu^2 }\right) + \lambda \bigg)}_{\triangleq b(\lambda, \nu^2) } \nonumber.
    \end{align}
    The function $a(\lambda, \nu^2)$ is negative since $\lambda\geq 0$ and $  \nu> 0 $. Next, the logarithm bound $\ln(r) \geq 1 - 1/r $ ensures that: 
    \begin{align}
        b(\lambda, \nu^2) \geq \sigma^2 \left( 1 - \frac{\lambda + \nu^2}{\nu^2}\right) + \lambda = 0.  
    \end{align}
    Thus $\Delta(\lambda, \nu^2)$ is monotonically decreasing with respect to $\nu^2$, so we can use the assumption $\sigma^2 \leq \rho \lambda$ to lower bound $\Delta$: 
    \begin{align}
        \Delta(\lambda, B, \nu) & \geq % \Delta(\lambda, B, \sqrt{\rho \lambda})  = 
        % & = 1 - \frac{\lambda}{M} - e^{\lambda\left(\ln\left[\left(\frac{c}{c+1}\right)^{(1 + c)}\right] + 1\right)} \\
        1 - \frac{\lambda}{B} - e^{\lambda \varphi  } \triangleq \Delta_1(\lambda, B) \nonumber 
    \end{align}
    where $\varphi  \triangleq \scriptscriptstyle \ln\left[\left(\frac{\rho}{\rho+1}\right)^{(1 + \rho)}\right] + 1$. 
    
    Next, we wish to show that $\Delta_1(\lambda, B)\geq 0 $ for $\lambda \in [0,B-1]$. %Given the assumptions that $B \geq W_{-1}(\varphi e^\varphi) / \varphi, \lambda \in [0, B-1]$ and $\rho >0$, 
    We will prove this by showing that $\Delta_1(\lambda, B) \geq 0 $ for $\lambda = \{ 0, B-1\} $ and $\Delta_1$ is concave with respect to $\lambda$. %and then applying definition of concave functions. 

    % \begin{enumerate}
    \noindent \underline{\textbf{(1)} At $\lambda = 0 $:} \quad \quad  $\Delta_1(0, B, \rho) & = 1 - 0 - e^0 = 0$
    \noindent\underline{\textbf{(2)}   At $\lambda = B-1$:} 
    \begin{align}
          \Delta_1(B-1, B , \rho) & = \frac{1}{B}- e^{(B-1)\varphi} \triangleq \Psi_\varphi(B) \geq 0 .  
    \end{align} 
    Since we assumed that $\varphi e^\varphi \in [-e^{-1}, 0)$ and $B \geq \frac{W_{-1}(\varphi e^\varphi)}{\varphi}$, we apply Lemma \ref{lem:lambert} to find that $\Psi_\varphi(B) \geq 0 $. %To ensure nonnegativity at this value of $\lambda$, we use the Lambert $W$-function to solve for $B_*$ such that $\Delta_2(B_*, \rho) = 0 $. This occurs at $B_* = \frac{W_i(\varphi e^\varphi)}{\varphi}$. Since $\varphi $ is real-valued, we only need to consider $i=0$ (where $B_{*,0} = 1$)  and $i=-1$.
    \noindent \underline{\textbf{(3)} Concavity for $\lambda \in [0, B-1]$:}
    Consider the second derivative of $\Delta_1$ with respect to $\lambda$, 
        % \begin{align}
            $\frac{\partial^2  \Delta_1}{\partial \lambda^2} & = -\varphi^2 e^{\lambda \varphi} \leq 0. $
        % \end{align}
        Thus $\Delta_1$ is concave with respect to $\lambda.$ 
        Since $\Delta_1(0, B)\geq 0$ and $\Delta_2(B-1, B) \geq 0 $, concavity of $\Delta_1(\lambda , B, \rho)$ ensures that $\Delta_1(\lambda , B, \rho) \geq 0 $ for all $\lambda \in [0, B-1].$
    % \end{enumerate} 
    %Since $\Delta_1(\lambda, M) $ is greater than or equal to zero at $\lambda = 0$ and $\lambda = B-1$ and that it is concave, it must also be nonnegative for all $\lambda \in [0, M-1]$.  

    \noindent Using this lower bound for $\Delta_1(\lambda, B) $, we have
    $\Delta(\lambda, M, \sigma) \geq \Delta_1(\lambda, B) \geq 0 $
    which implies the desired inequality \eqref{eq:comparison_thm}.%, $H(\lambda ,\sigma) \leq 1 - \frac{\lambda}{B}$.
\end{proof}


==> extended_proofs/lambert_info.tex <==
\begin{definition}[Lambert $W$-function on $\R$ \cite{corless1996lambert}]
    $W_i: \mathbb{R} \to \mathbb{R}$ where  $z = W_i(z)e^{W_i(z)}$ for $ i =\{ 0, -1\}.$ 
\end{definition}

\noindent Important properties of the Lambert-$W$ function \cite{corless1996lambert} include: 
\begin{enumerate}
    \item If $z \in [-e^{-1}, 0)$, then $W_{-1}(z) $ exists,   
    \item When they both exist $W_0(z) \geq -1 \geq  W_{-1}(z)$.
\end{enumerate}


==> extended_proofs/lambert_lemma.tex <==



\begin{lemma} \label{lem:lambert}
    Let $W_i$ be the Lambert-$W$ function. If $\Psi_\varphi(B) = \frac{1}{B}- e^{(B-1)\varphi}$
    for some $\varphi \in \R$ such that $\varphi e^\varphi \in [- e^{-1}, 0)$, then $\Psi(B) \geq 0 $ for all $B \geq \frac{W_{-1}(\varphi e^\varphi)}{\varphi}$.
\end{lemma}
\begin{proof}
    The zeros of $\Psi_\varphi$ are $B_i=  \frac{W_i(\varphi e^\varphi)}{\varphi}$ for $i = \{ 0, -1 \}$. Since $\varphi e^\varphi \in [-e^{-1}, 0)$,  it follows from the properties of $W_i$ that $B_{-1} $ exists and that $B_{-1} \geq B_0$. 
    
    First we show that $\Psi_\varphi$ has a nonnegative derivative at  $B_{-1}$:  
    \begin{align}
        \frac{d \Psi_\varphi}{d B}(B_{-1}) & = - \frac{1}{B_{-1}^2} - \varphi e^{(B_{-1} -1 )\varphi}  = - \frac{1}{B_{-1}^2} - \frac{\varphi}{B_{-1}}\\
        & = -\frac{1}{B_{-1}^2} - \frac{W_{-1}(\varphi e^\varphi)}{B_{-1}^2 } \geq \frac{-1 + 1}{B_{-1}^2}= 0 . \nonumber
    \end{align}
    Where we used the properties of the Lambert-$W$ function which ensure that $B_{-1}$ is a zero of $\Psi_\varphi$ and $-W_{-1}(\varphi e^\varphi) \geq 1$. 
    
    Since $B_{-1}$ is the largest zero of $\Psi_\varphi$, $\frac{d\Psi_\varphi}{d B}(B_{-1}) \geq  0 $, and $\Psi_\varphi(B)$ is continuous and well defined for $B \geq B_{-1}$, we find that $\Psi_\varphi(B) > 0 $ for all $B > B_{-1}$. 
\end{proof}

==> extended_proofs/new_cmart_proof.tex <==


\begin{proof}
    First we define the normalized safety function
    \begin{align}
        \eta(\mb{x}) \triangleq h(\mb{x}) / \delta 
    \end{align}
    to ensure that the martingale differences will be bounded by 1. We then use $\eta$ to define the  candidate supermartingale $\mart_k = -\eta(\mb{x}_k)  - \frac{kc}{\delta}+ \eta(\mb{x}_0) $, which satisfies $\mart_0 = 0 $ and is a supermartingale: 
    \begin{align}
        \E[\mart_{k+1}~|~ \F_k] & = \E[-\eta(\mb{x}_{k+1})|\F_k] - (k+1)\frac{c}{\delta} + \eta(\mb{x}_0) \nonumber  \\
        & \leq -\eta(\mb{x}_k) - k\frac{c}{\delta} + \eta(\mb{x}_0)  = \mart_k .
    \end{align}
    Consider the Doob's decomposition of this supermartingale. The resulting martingale is: 
    \begin{align}
        M_k & = \mart_k - \sum_{i=1}^k (\E[\mart_i ~|~ \F_{i-1}] - \mart_{i-1} )\\
        & = \mart_k + \sum_{i=1}^k\left(\E [\eta_i | \F_{i-1} ] - \eta_{i-1} + \frac{c}{\delta} \right) \geq \mart_k 
    \end{align}
    The martingale difference is given by: 
    \begin{align}
        M_{k} - M_{k-1} &= \mart_k - \E[\mart_{k} ~|~ \F_{k-1}]\\
        & = -\eta(\mb{x}_k) +  \E[\eta(\mb{x}_k) ~|~ \F_{k-1}] \leq \frac{\delta}{\delta} = 1 
    \end{align}
    Finally, we must ensure that $\langle M \rangle_K$ is bounded:
    \begin{align}
        \langle M \rangle_K &= \sum_{i=1}^K \E[(M_i - \E[M_i | \F_{i-1}])^2 | \F_{i-1}]\\
        & = \sum_{i=1}^K \frac{1}{\delta^2}\textup{Var}(h(\mb{x}_{i})| \F_{i-1})\leq K\frac{\sigma^2}{\delta^2}  
    \end{align}
    Now we consider the inequalities: 
    \begin{align}
        & \max_{k \leq K } -\eta(\mb{x}_k) - K\frac{c}{\delta} + \eta(\mb{x}_0)  \leq \max_{k \leq K } \eta(\mb{x}_k) - k\frac{c}{\delta} + \eta(\mb{x}_0) \nonumber \\
        & = \max_{k \leq K } \mart_k \leq \max_{k \leq K }M_k .
    \end{align}
    Consider the case when $\lambda^* = -K\frac{c}{\delta} +\eta(\mb{x}_0)$. Then the safety event satisfies the containment:  
    \begin{align}
        & \left\{\min_{k \leq K } h(\mb{x}_k) < 0  \right\} \subset \left\{ \max_{k \leq K } \mart_k \geq \lambda^* \right\} \subseteq \left \{ \sup_{k \leq K } M_k \geq \lambda^*  \right\}. \nonumber 
    \end{align}
    Applying the probability bound from Theorem \ref{thm:azuma_hoeffding} results in the desired probability bound: 
    \begin{align}
        & P_u(K, \mb{x}_0) \leq H\left(\frac{-Kc + h(\mb{x}_0)}{\delta},\frac{\sigma\sqrt{K}}{\delta} \right)
    \end{align}
    %Finally, since we know, almost surely, that the system cannot leave the set within $h(\mb{x}_0)/c$ steps, we can further strengthen this probability by changing the event in the indicator function from $\mathds{1}_{\{h_0 /(1 + c) \leq K \}}$ to $\mathds{1}_{\{h_0 /c \leq K \}}. $
\end{proof}


==> extended_proofs/stoch_issf_proof.tex <==



\begin{proof}
    First define $\eta(\mb{x}) = \frac{h(\mb{x}) + \epsilon}{\delta}$ and $\mart_k = -\alpha^{K-k}\eta(\mb{x}_k) + \alpha^K \eta(\mb{x}_0) + \sum_{i=1}^k\alpha^{K-i} \frac{\epsilon}{\delta} (1 - \alpha)$. First note that $h_k$ satisfies: 
    \begin{align}
        E[\eta(\mb{x}_k) | \F_{k-1}] \geq \alpha (\eta_{k-1}) + \frac{\epsilon}{\delta} (1 - \alpha )
    \end{align}
    
    Note that $\mart_k$ satisfies $\mart_0 = 0 $ and is a supermartingale: 
    \begin{align}
        & \E[\mart_{k+1}|\F_{k} ] \\
        & = -\alpha^{K-(k+1)}\E[\eta_{k+1} | \F_k ] + \alpha^K \eta_0 + \sum_{i=1}^{k+1} \alpha^{K-i} \epsilon (1 - \alpha) /\delta  \nonumber \\
        & \leq -\alpha^{K-k}\eta_k + \alpha^K \eta_0+ \sum_{i=1}^{k} \alpha^{K-i} \epsilon ( 1- \alpha)/\delta  = \mart_k. 
    \end{align}

    Next, we take the Doob's decomposition and consider the martingale: 
    \begin{align}
        M_k & = \mart_k + \sum_{i=1}^k (\mart_{i-1}  - \E[\mart_i|\F_{i-1}] )\\
        & = R_k + \sum_{i=1}^k\alpha^{K-i}\left(\E[\eta(\mb{x}_i)|\F_{i-1}] - \alpha \eta_{i-1} + \frac{\epsilon}{\delta}(1-\alpha)\right) \nonumber \\
        & \leq R_k 
    \end{align}
    
    Since the predictable quadratic variation $\langle h(\mb{x}) \rangle_k $ is bounded, so is $\langle M \rangle_k$: 
    \begin{align}
        \langle M \rangle_k & = \sum_{i=1}^k \E[(W_i - \E[W_i | \F_{i-1}])^2 |\F_{i-1}]\\
        & = \sum_{i=1}^k \alpha^{2(K-i)}\E[(\eta(\mb{x}_k ) -  \E[\eta(\mb{x}_i) | \F_{i-1}])^2| \F_{i-1}]\\
        & = \sum_{i=1}^k \frac{\alpha^{2(K-i)}}{\delta^2} \E[(h(\mb{x}_k) - \E[h(\mb{x}_i)  | \F_{i-1}])^2|\F_{i-1}]\\
        & \leq \sum_{i=1}^k \frac{\alpha^{2(K-i)}}{\delta^2} \sigma^2 \leq \frac{K \sigma^2}{\delta^2}
    \end{align}
    Next we consider the implications:
    \begin{align}
        & \min_{k \leq K } \eta(\mb{x}_k) < 0 \implies \min_{1 \leq k \leq K } \eta(\mb{x}_k) \leq 0 \\
        &  \implies  \max_{1 \leq k \leq K }W_k \geq  \alpha^K \eta(\mb{x}_0)  \implies  \max_{1 \leq k \leq K }M_k \geq  \alpha^K \eta(\mb{x}_0) \nonumber
    \end{align}
    Considering the case when $\lambda^* = \alpha^K \eta(\mb{x}_0) $ ensures that: 
    \begin{align}
        P_u(K, \mb{x}_0) \leq H\left(\alpha^K \eta(\mb{x}_0), \frac{\sigma\sqrt{k}}{\delta}\right) \label{cor_pf:freedman}
    \end{align}
    Finally we can bound $h$ as in Proposition \ref{thm:issf} to find that: 
    \begin{align}
        h(\mb{x}_k) \geq \alpha^K h(\mb{x}_0) - \sum_{i=0}^{K-1}\alpha^i \delta \quad \textup{(a.s.)}
    \end{align} to achieve the indicator probability: 
    \begin{align}
        P_u(K, \mb{x}_0) \leq \mathds{1}_{\left \{ -\epsilon \geq \alpha^K h(\mb{x}_0) - \sum_{i=0}^{K-1} \alpha^i \delta \right \} } \label{cor_pf:indicator}
    \end{align} and take the smaller bound between \eqref{cor_pf:freedman} and \eqref{cor_pf:indicator} via multiplication, to obtain the desired bound in \eqref{eq:p_issf_bound}.
\end{proof}

